GeoMix: Descriptor-Free Visual Localization via Global Context and Multi-Detector Training

Descriptor-free visual localization eliminates high-dimensional descriptor storage, preserves scene privacy, and simplifies map maintenance, yet its accuracy still lags far behind descriptor-based pipelines. We identify this gap to insufficient geometric discriminability in geometry-only matching. Without visual appearance, current methods underutilize local geometry cues, lack the global context among keypoints, and overfit to a single keypoint detector. We further observe that descriptor-free matching naturally enables multi-detector training, as heterogeneous keypoints can be optimized in a shared geometry-only space without aligning descriptor spaces. Building on these insights, we propose GeoMix, a descriptor-free 2D-3D matching framework that strengthens geometric discriminability at three levels. Locally, directional and distance-aware embeddings enrich neighborhood aggregation with fine-grained spatial structure. Globally, learnable context nodes aggregate and redistribute scene-wide information via cross-attention to resolve ambiguities beyond local receptive fields. At the training level, Mix-Training exploits this detector-agnostic geometry space to learn representations across multiple keypoint detectors. Extensive experiments on MegaDepth, Cambridge Landmarks, 7Scenes, and Aachen Day-Night show that GeoMix sets a new state of the art among descriptor-free methods, reducing 75th-percentile rotation error by 89\% and translation error by up to 90\% over the previous best, while generalizing zero-shot to unseen detectors and narrowing the gap to descriptor-based pipelines. Code is available at $\href{https://github.com/YejunZhang/Geomix}{\text{this links}}$.

==> figures/global_context.tex <==
% Preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows.meta,calc,positioning,fit}

\begin{tikzpicture}[
    x=1cm, y=1cm,
    % --- Shared dimensions ---
    frame w/.initial=6cm,   frame h/.initial=4.2cm,
    box w/.initial=5.4cm,   box h/.initial=1.5cm,
    % --- Frame styles ---
    innerframe/.style={
        draw=black, rounded corners=6pt, line width=1.1pt,
        fill=white, inner sep=0pt,
        minimum width=\pgfkeysvalueof{/tikz/frame w},
        minimum height=\pgfkeysvalueof{/tikz/frame h}
    },
    dashedbox/.style={
        draw=black, dashed, line width=0.9pt, inner sep=0pt,
        minimum width=\pgfkeysvalueof{/tikz/box w},
        minimum height=\pgfkeysvalueof{/tikz/box h}
    },
    gcsel/.style={
        draw=red!70!black, dashed, rounded corners=2pt,
        line width=1.0pt, inner sep=0pt,
        minimum width=0.8cm, minimum height=0.8cm, anchor=center
    },
    % --- Base circle + color variants ---
    basenode/.style={
        circle, draw=black!80, minimum size=0.48cm,
        line width=0.8pt, inner sep=0pt, anchor=center
    },
    gnode/.style={basenode, fill=green!45},
    onode/.style={basenode, fill=orange!90},
    pnode/.style={basenode, fill=violet!35},
    penode/.style={basenode, fill=orange!20},
    % --- Connection styles ---
    conn/.style={line width=0.9pt},
    gcconn/.style={line width=0.9pt, black},
]

% ================================================================
% Helper: draw one frame with title, two dashed boxes, and 8 nodes
%   #1 = frame name prefix (L / R)
%   #2 = anchor coordinate
%   #3 = title text
% ================================================================
\newcommand{\drawframe}[3]{%
    \node[innerframe, anchor=center] (#1F) at (#2) {};
    \node[font=\large\bfseries, anchor=center] at ($(#1F.north)+(0,0.2)$) {#3};
    % Upper / lower dashed boxes
    \node[dashedbox, anchor=center] (#1FUpperBox) at ($(#1F.center)+(0, 1.1)$) {};
    \node[dashedbox, anchor=center] (#1FLowerBox) at ($(#1F.center)+(0,-1.1)$) {};
    % Upper row: 3 green + 1 orange
    \foreach \i/\xoff in {1/-1.8, 2/-0.6, 3/0.6}{
        \node[gnode] (#1UG\i) at ($(#1FUpperBox.center)+(\xoff, 0.25)$) {};
    }
    \node[onode] (#1UO) at ($(#1FUpperBox.center)+(1.8, 0.25)$) {};
    % Lower row: 3 purple + 1 peach
    \foreach \i/\xoff in {1/-1.8, 2/-0.6, 3/0.6}{
        \node[pnode] (#1LP\i) at ($(#1FLowerBox.center)+(\xoff,-0.25)$) {};
    }
    \node[penode] (#1LPe) at ($(#1FLowerBox.center)+(1.8,-0.25)$) {};
}

% ================================================================
% Draw both frames
% ================================================================
\drawframe{L}{0,0}{Self(knn)}
\drawframe{R}{7,0}{Cross}

% ================================================================
% Self(KNN) connections: chains + arcs
% ================================================================
% Upper chain (regular) + GC link
\draw[conn] (LUG1) -- (LUG2) -- (LUG3);
\draw[gcconn] (LUG3) -- (LUO);
% Arcs from orange GC node to each green (bend downward)
\foreach \i/\b in {1/35, 2/22, 3/12}{
    \draw[gcconn, bend left=\b] (LUO.south) to (LUG\i.south);
}
% Lower chain (regular) + GC link
\draw[conn] (LLP1) -- (LLP2) -- (LLP3);
\draw[gcconn] (LLP3) -- (LLPe);
% Arcs from peach GC node to each purple (bend upward)
\foreach \i/\b in {1/35, 2/22, 3/12}{
    \draw[gcconn, bend right=\b] (LLPe.north) to (LLP\i.north);
}

% ================================================================
% Cross connections: fully connected upper <-> lower
% ================================================================
% Regular nodes to regular nodes
\foreach \U in {RUG1, RUG2, RUG3}{
    \foreach \L in {RLP1, RLP2, RLP3}{
        \draw[conn] (\U.south) -- (\L.north);
    }
}
% GC node connections (orange color)
\foreach \L in {RLP1, RLP2, RLP3, RLPe}{
    \draw[gcconn] (RUO.south) -- (\L.north);
}
\foreach \U in {RUG1, RUG2, RUG3}{
    \draw[gcconn] (\U.south) -- (RLPe.north);
}

% ================================================================
% GC node highlights
% ================================================================
\node[gcsel] (GCBoxU) at (LUO.center) {};
\node[gcsel] (GCBoxL) at (LLPe.center) {};
\node[gcsel] at (RUO.center) {};
\node[gcsel] at (RLPe.center) {};
\node[font=\normalsize, text=red!70!black, anchor=center] (GCLabel)
    at ($(LUO.south)!0.5!(LLPe.north)+(-0.2,0)$) {GC Nodes};
\draw[-{Stealth[length=4pt]}, red!70!black, line width=0.8pt] (GCLabel.north) to[bend right=30] (GCBoxU.south);
\draw[-{Stealth[length=4pt]}, red!70!black, line width=0.8pt] (GCLabel.south) to[bend left=30] (GCBoxL.north);


% Add explicit bottom breathing room in the picture bounding box.
\path[use as bounding box]
    ($(current bounding box.south west)+(0,-0.2)$)
    rectangle
    (current bounding box.north east);

\end{tikzpicture}


==> figures/local_geo_encoding.tex <==
% Preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows.meta,calc,positioning,shapes.geometric}

\begin{tikzpicture}[
    x=1cm,y=1cm,
    % --- Global styles ---
    arr/.style={draw=black, line width=1pt, -{Stealth[length=3.5mm,width=3mm]}},       % arrow style used for all connections
    line/.style={draw=black, line width=1pt},                                            % basic line style
    box/.style={line, fill=white, rounded corners=3.5mm},                                % rounded white box (container)
    rowbox/.style={box, minimum width=1.35cm, minimum height=0.50cm},                    % unused; kept for potential row-level boxes
    dot/.style={circle, inner sep=0pt, minimum size=0.36cm, line width=0.9pt},           % base dot style for colored points
    % NOTE: dblue is defined twice; the second definition (line 15) overrides the first
    dblue/.style={dot, draw=blue!55!black, fill=blue!20},                                % blue dot (overridden below)
    dyellow/.style={dot, draw=orange!75!black, fill=yellow!30},                          % yellow dot
    dpurple/.style={dot, draw=violet!55!black, fill=violet!20},                          % purple dot
    dblue/.style={dot, draw=blue!75!black, fill=blue!30},                                % blue dot (this overrides the earlier dblue)
    dgreen/.style={dot, draw=green!75!black, fill=green!30},                             % green dot
    dorange/.style={dot, draw=orange!75!black, fill=orange!30},                          % orange dot
    dred/.style={dot, draw=red!75!black, fill=red!30},                                   % red dot
    cdot/.style={circle, line width=1pt, minimum size=0.42cm},                           % plain circle dot (used for output node)
    smlabel/.style={font=\small, align=center},                                          % small centered label for edge annotations
    biglabel/.style={font=\huge},                                                        % large label (unused)
]

% =====================================================================
% (Optional title – currently commented out)
% =====================================================================
% \node[font=\bfseries\fontsize{22}{24}\selectfont] at (6.85,2.10) {Self-Attention};

% =====================================================================
% 1. INPUT POINT  →  KNN Search  →  NEIGHBORS BOX
%    A single query point on the left; arrow labeled "KNN Search"
%    leads to a box holding a 3×2 grid of colored neighbor dots.
% =====================================================================
\node[circle, box, minimum size=0.36cm, anchor=center] (in) at (-1,-1) {};          % query point (small circle)
\node[box, minimum width=1.2cm, minimum height=1.70cm, anchor=center] (nbr) at ($(in.center)+(2,0)$) {};  % neighbor container
\node[font=\large, anchor=center] at ($(nbr.north)+(0,0.25)$) {Neighbors};            % label above neighbor box
\draw[arr] (in.east) -- (nbr.west) node[midway, above=-11pt, smlabel] {KNN\\Search};  % arrow: input → neighbors

% 3×2 grid of colored dots inside the neighbor box
\foreach \x/\y/\s in {
  -0.45/ 0.50/dblue,   0.05/ 0.50/dyellow,
  -0.45/ 0.00/dpurple, 0.05/ 0.00/dblue,
  -0.45/-0.50/dyellow, 0.05/-0.50/dpurple}
  \node[\s,anchor=west] at ($(nbr.center)+(\x,\y)$) {};

% =====================================================================
% 2. NEIGHBORS  →  Extract Priors  →  PRIORS BOX
%    Arrow labeled "Extract priors" connects neighbor box to a wider
%    box that shows (dots + angle symbols), representing geometric
%    priors (distances ↔ and angles ∠) extracted from the neighbors.
% =====================================================================
\node[box, minimum width=2.2cm, minimum height=1.7cm, anchor=center] (pri) at ($(nbr.east)+(2.4,0)$) {};  % priors container
\draw[arr] (nbr.east) -- (pri.west) node[midway, above=-11pt, smlabel] {Extract\\priors};                  % arrow: neighbors → priors

% Left column of colored dots inside the priors box (shifted left by extra -0.45)
\foreach \x/\y/\s in {
  -0.45/ 0.50/dblue,   0.05/ 0.50/dyellow,
  -0.45/ 0.00/dpurple, 0.05/ 0.00/dblue,
  -0.45/-0.50/dyellow, 0.05/-0.50/dpurple}
  \node[\s,anchor=west] at ($(pri.center)+(\x -0.45 ,\y)$) {};

% Right column: distance–angle symbols (↔∠) next to each row of dots
\foreach \yy in {0.5,0.00,-0.5}
  \node[anchor=center, font=\large]
    at ($(pri.center)+(0.55,\yy)$) {$\leftrightarrow\hspace{-0.3pt}\angle$};

% =====================================================================
% 3a. UPPER BRANCH: Priors  →  Maxpooling  →  Global feature (gray dot)
%     Aggregates the prior features via max-pooling into a single
%     global descriptor (gray circle on the right).
% =====================================================================
\node[box, minimum height=0.5cm, anchor=west] (maxp) at ($(pri.east)+(1,+1)$) {{\fontsize{14.4}{18}\selectfont Maxpooling}
};  % maxpooling box
\draw[arr] (pri.east) -- (maxp.west);                                                                 % arrow: priors → maxpooling

\node[cdot, draw=teal!75!black, fill=teal!30, anchor=center] (gTop) at ($(maxp.east)+(1,0)$) {};           % global feature output dot
\draw[arr] (maxp.east) -- (gTop.west);                                                                 % arrow: maxpooling → output dot

% =====================================================================
% 3b. SECTION LABEL: "Angular Convolution"
%     Placed between the two branches for visual reference.
% =====================================================================
\node[minimum height=0.5cm, anchor=center] (ang) at ($(maxp.west)+(+1.9,-3.3)$) {\large Annular Convolution};
% (Commented-out alternative styling for the label)
% \node[anchor=base west, biglabel, fill=violet!20,
%       rounded corners=1pt, inner xsep=2pt, inner ysep=1pt]
  % at ($(ang.base east)+(0.15,0)$) {Convolution};

% =====================================================================
% 3c. LOWER BRANCH: Priors  →  Angular Convolution block  →  Output dots
%     The angular convolution groups neighbors by similar angles,
%     producing a condensed set of per-angle features (3 colored dots).
% =====================================================================
\node[box, minimum width=2.2cm, minimum height=1.91cm, anchor=west] (ac) at ($(pri.east)+(1,-1)$) {};  % angular conv container
\draw[arr] (pri.east) -- (ac.west) node[midway, below=-5pt, sloped, smlabel] {Group};                         % arrow: priors → angular conv

% Sub-boxes around each row pair of dots
\foreach \yy in {0.55, 0.00, -0.55}
  \node[line, fill=white, minimum width=1.05cm, minimum height=0.45cm, anchor=center]
    at ($(ac.center)+(-0.45,\yy)$) {};

% Dots inside angular conv box – note same-color pairs per row
% (neighbors have been grouped by angular similarity)
\foreach \x/\y/\s in {
  -0.45/ 0.55/dblue,   0.05/ 0.55/dblue,
  -0.45/ 0.00/dpurple, 0.05/ 0.00/dpurple,
  -0.45/-0.55/dyellow, 0.05/-0.55/dyellow}
  \node[\s,anchor=west] at ($(ac.center)+(\x -0.45 ,\y)$) {};


\foreach \yy in {0.55, 0.00, -0.55}
  \node[line, fill=white, minimum width=0.8cm, minimum height=0.45cm, anchor=center]
    at ($(ac.center)+(0.55,\yy)$) {};

% Distance–angle symbols next to each row
\foreach \yy in {0.55,0.00,-0.55}
  \node[anchor=center, font=\large]
    at ($(ac.center)+(0.55,\yy)$) {$\leftrightarrow\!\angle$};

% Narrow output column: 3 aggregated feature dots (red, green, orange)
\node[box, minimum width=0.6cm, minimum height=1.8cm, anchor=east ] (col) at ($(ac.east)+(1.2,0)$) {};  % output column box
\draw[arr] (ac.east) -- (col.west);                                                                       % arrow: angular conv → output

% Three output dots representing per-angle aggregated features
\foreach \y/\s in {0.50/dred, 0.00/dgreen, -0.50/dorange}
  \node[\s,anchor=center] at ($(col.center)+(0,\y)$) {};

% Output dot for the lower branch (mirroring gTop in the upper branch)
\node[cdot, draw=orange!75!black, fill=orange!30, anchor=center] (gBot) at (gTop |- col.east) {};
\draw[arr] (col.east) -- (gBot.west);

% Vertical line connecting gTop and gBot, with midpoint branching to merge node
\draw[line] (gTop.south) -- (gBot.north);
\coordinate (mid) at ($(gTop.south)!0.5!(gBot.north)$);
\node[cdot, draw=pink!75!black, fill=pink!30, anchor=center] (merge) at ($(mid)+(1.2,0)$) {};
\draw[arr] (mid) -- (merge.west) node[near start, above, font=\large] {$+$};

\end{tikzpicture}


==> figures/mix_training.tex <==
\begin{tikzpicture}[
    x=1cm, y=1cm,
    arr/.style={->, >=Stealth, line width=0.8pt, color=black!70},
    imgbox/.style={
        draw=black!45, rounded corners=2pt, fill=white,
        inner sep=2pt, line width=0.7pt
    },
    panel/.style={
        draw=black!35, rounded corners=3pt, fill=clrGrayBg,
        inner sep=4pt, line width=0.7pt
    },
    det/.style={
        draw=#1!85!black, rounded corners=2pt, fill=#1!12,
        minimum width=1.6cm, minimum height=0.2cm,
        align=center, font=\scriptsize\bfseries, line width=0.8pt
    },
    model/.style={
        draw=black!45, rounded corners=3pt, fill=white,
        minimum width=1.5cm, minimum height=0.8cm,
        align=center, font=\scriptsize, line width=0.7pt
    },
    outbox/.style={
        draw=clrOrange!75!black, rounded corners=3pt, fill=clrOrange!10,
        minimum width=2.1cm, minimum height=0.72cm,
        align=center, font=\scriptsize\bfseries, line width=0.9pt
    }
]

% ── Query image branch ────────────────────────────────────────────────────────
\node[imgbox, minimum width=1cm, minimum height=0.5cm,
      align=center, font=\scriptsize, text=black]
    (query) at (0, 0.2) {Query\\Image};

% ── Detector pool ─────────────────────────────────────────────────────────────
\node[panel, anchor=west, minimum width=1.5cm, minimum height=1.5cm]
    (pool) at ([xshift=0.75cm]query.east) {};
\node[font=\tiny, text=black, anchor=north]
    at ([yshift=4pt]pool.north) {Detector};

\node[det=clrBlue,   anchor=north, minimum width=1.2cm, minimum height=0.15cm,
      font=\tiny] (sift) at ([yshift=-0.4cm]pool.north) {SIFT};
\node[det=clrOrange, below=0.06cm of sift,
      minimum width=1.2cm, minimum height=0.15cm, font=\tiny] (sp)   {SuperPoint};
\node[det=clrGreen,  below=0.06cm of sp,
      minimum width=1.2cm, minimum height=0.15cm, font=\tiny] (disk) {DISK};

\draw[arr] (query.east) -- (pool.west);

% ── Fixed 3D branch ───────────────────────────────────────────────────────────
\node[imgbox, anchor=north, minimum width=1cm, minimum height=0.5cm,
      align=center, font=\scriptsize, text=black]
    (map) at ([yshift=-0.6cm]query.south) {Point\\Cloud};

\node[draw=black!35, rounded corners=3pt, fill=clrGrayBg,
      anchor=north, minimum width=2.2cm, minimum height=0.2cm,
      align=center, font=\scriptsize, line width=0.8pt]
    (fixdet) at ([yshift=-0.3cm]pool.south) {Fixed 3D Points};

\draw[arr] (map.east) -- (fixdet.west);

% ── Vertical midpoint ─────────────────────────────────────────────────────────
\coordinate (midqm) at ($(query.center)!0.5!(map.center)$);

% ── Form Training Pairs ───────────────────────────────────────────────────────
\node[draw=black!45, rounded corners=2pt, fill=white,
      minimum width=1.5cm, minimum height=1.1cm, line width=0.7pt,
      align=center, font=\tiny, anchor=center]
    (pairs) at ([xshift=2cm, yshift=0.15cm]pool.east |- midqm)
    {\textbf{Training}\\
     \textbf{Pairs}\\[2pt]
     \begin{tabular}{@{}l@{}}
     {\color{clrBlue!80!black}$\bullet$} SIFT\,+\,3D\\[-1pt]
     {\color{clrOrange!85!black}$\bullet$} SP\,+\,3D\\[-1pt]
     {\color{clrGreen!80!black}$\bullet$} DISK\,+\,3D
     \end{tabular}};

% ── Arrows: detectors + 3D → pairs ───────────────────────────────────────────
\draw[arr, dashed, clrBlue!80!black]   (sift.east)   -- (pairs.west);
\draw[arr, dashed, clrOrange!85!black] (sp.east)     -- (pairs.west);
\draw[arr, dashed, clrGreen!80!black]  (disk.east)   -- (pairs.west);
\draw[arr] (fixdet.east) -- ([yshift=-0.25cm]pairs.west);

% ── GeoMix Network ────────────────────────────────────────────────────────────
\node[model, anchor=west, draw=clrBlue!70, fill=clrBlueBg, line width=1.0pt]
    (shared) at ([xshift=0.55cm]pairs.east) {GeoMix\\Network};

% Arrow: pairs → model
\draw[arr] (pairs.east) -- (shared.west);

% Add explicit bottom breathing room in the picture bounding box.
\path[use as bounding box]
    ($(current bounding box.south west)+(0,-0.1)$)
    rectangle
    (current bounding box.north east);


\end{tikzpicture}
